Verifying Array Manipulating Programs by Tiling

Formally verifying properties of programs that manipulate arrays in loops is computationally challenging. In this paper, we focus on a useful class of such programs, and present a novel property-driven verification method that first infers array access patterns in loops using simple heuristics, and then uses this information to compositionally prove universally quantified assertions about arrays. Specifically, we identify tiles of array accesses patterns in a loop, and use the tiling information to reduce the problem of checking a quantified assertion at the end of a loop to an inductive argument that checks only a slice of the assertion for a single iteration of the loop body. We show that this method can be extended to programs with sequentially composed loops and nested loops as well. We have implemented our method in a tool called Tiler. Initial experiments show that Tiler outperforms several state-of-the-art tools on a suite of interesting benchmarks.

==> alg-daikon.tex <==
\begin{algorithm}[!t]
 \caption{\textsc{Program Transformation for Daikon}}
 \label{alg:instdaikon}
\begin{algorithmic}[1]
  \Require Program $P$ with a main, set ${\tile_a}$ of tiles for $a \in P$, set $Inputs$ of variables read before written
  \State Fix size of all arrays in main to \texttt{SMALLVAL}
  \ForAll{$a \in Inputs$}
    \Comment{Initialize arrays in main}
    \State for($i=0; i < size; i++$) { $a[i] = rand();$ }
  \EndFor
  \ForAll{$v \in Inputs$}
    \Comment{Initialize variables read before written in main}
    \State $v = rand();$
  \EndFor

  \ForAll{loops $l \in P$}
%   \State Create a map $map$ between string representations of $a[iExpr]$ and scalar variable representing it
  \ForAll{$a \in P$}
    \ForAll{$\tile^k_a \in {\tile_a}$}
      \If {$|\tile^l_a| == |\tile^k_a|$}
        \ForAll{$iExpr \in \tile^k_a$}
          \Comment{Store in a map}
          \State Create new scalar variable $x$
          \State map[string($x$)]=string($a[iExpr]$)
        \EndFor
      \EndIf
    \EndFor
  \EndFor
  \ForAll{$v$ writes to or reads from $a$}
    \State Create new scalar variable $x$
    \State map[string($x$)] = string($v$)
  \EndFor

  \State Output - dummy\_l(
  \Comment Add dummy calls at end of body
  \ForAll{$key \in map$} $map[key]$);
  \EndFor
  \State Output - void dummy\_l(
  \Comment Create a empty function definition
  \ForAll{$key \in map$} $type(key)$ $key$)
  \EndFor
   \{ \}
\EndFor
  
\end{algorithmic}
\end{algorithm}


==> alg-instrument.tex <==
\begin{algorithm}[!t]
 \caption{\textsc{Instrument}($\program,\formula = \formula_{arith}
   \land \forall j. (lb' \leq j < ub' ) \limplies good(a[j]) $)}
 \label{alg:tiling}
\begin{algorithmic}[1]
  \State assuming a single array is involved
  \State introduce three fresh variables $i$, $j$, and $j\_old$ 
  \State $j\_old := UNINIT;j := UNINIT;i := 0$ inserted before the loop body
  \State $assert(j\_old \neq  UNINIT \land j \neq  UNINIT \limplies j\_old \neq j); i++; j\_old := j; j := UNINIT$
  is inserted just before the end of the loop body
  \State Every array access(read/write) ( $a[e] = ..$ or $.. = e'(a[e])$)
  to array is appended with $ if(NONDET) j := e$ 
  \State Each array write $a[e] = e'$ is replaced by $assert( good(e') )$ 
\end{algorithmic}
\end{algorithm}  

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> alg-tilegen.tex <==
\begin{algorithm}[!t]
  \caption{TileGen($\PP, \alpha, \beta$)}
  \label{alg:tilegen}
  \begin{algorithmic}[1]
    \Require Program $\PP = (\mathcal{V}, \mathcal{A}, \mathcal{L}, \Phi)$, $\alpha : \mathcal{L} \rightarrow \mathcal{E}$, $\beta : \mathcal{L} \rightarrow \mathcal{E}$  %, loop counter $i$ for $\LL$ takes values from $[\alpha_{\LL},\beta_{\LL}]$
    \Ensure $\Tile$ for each loop $\LL \in \mathcal{L}$ and array $\A \in \mathcal{A}$
    \For {each loop $\LL = for(k:=\EE;\mexit{\LL};k:=\EE) ~\{~ \LB ~\} \in \mathcal{L}$}
      \State Introduce fresh variables $i$ and $j_{\A}$ for each $\A \in \mathcal{A}$
      \State Create $\LL' = for(k:=\EE,i=0;\mexit{\LL};k:=\EE,i++) ~\{~ \LB' ~\} $ where $\LB'$ is such that each array write `$\A[\EE] = \EE'$' in $\LB$ is replaced with `$nondet(j_{\A}=\EE)$'
%      \State \mbox{}\hspace{3ex} increment $i'$ at the end of $\LB$
    \State $\mathsf{I} := AbstractInterpreter(\LL')$
    \For {each array $\A \in \mathcal{A}$}
      \State $\Tile_{\LL,\A}(i,j_{\A}) := Project(\mathsf{I}, i, j_{\A})$
%    \If {$i$ updated in body of $l$}
%      \State continue
%    	\EndIf
%    \State $lb(i) := \forall n. min(e^a_n(i))$
%    \State $ub(i) := \forall n. max(e^a_n(i))$
%    \State $\tile^l_a(i, j) := lb \leq j \leq ub$
      \State $\phi_d := i \neq i' \land \Tile(i,j_{\A}) \land \Tile(i',j_{\A})$
%    \Comment{Disjoint}
      \State $\phi_c := \Tile_{\LL,\A}(i,j_{\A}') \land \Tile_{\LL,\A}(i+1,j_{\A}'') \land j_{\A}' < j_{\A} < j_{\A}'' \land \lnot \Tile_{\LL,\A}(i,j_{\A}) \land \lnot \Tile_{\LL,\A}(i+1,j_{\A})$
%    \Comment{Compact}
%    \State $\phi_r := j' < j < j'' \land \Tile(k,j') \land \Tile(k,j'') \land \lnot \Tile(k,j)$
%    \Comment{Range like}
      \State $\gamma_{\A} := min ~\{~ j_{\A} : \Tile_{\LL,\A}(\alpha_{\LL}, j_{\A}) = \ltrue ~\}$
      \State $\delta_{\A} := max ~\{~ j_{\A} : \Tile_{\LL,\A}(\beta_{\LL}, j_{\A}) = \ltrue ~\}$
      \State $\phi_{lb} := \Tile_{\LL,\A}(\alpha_{\LL}, \gamma_{\A})$
      \State $\phi_{ub} := \Tile_{\LL,\A}(\beta_{\LL}, \delta_{\A})$

%    \State $\phi_{lb} := lb(0) \leq 0$
%    \Comment{Lower Bound}
%    \State $\phi_{ub} := exitCond(l) \limplies size(a) < ub(i)$
%    \Comment{Upper Bound}
      \If {$\neg (unsat(\phi_d) \land unsat(\phi_c) \land sat(\phi_{lb} \land \phi_{ub}))$}
%      \State $\Tile_a.add(\Tile^l_a)$
        \State Throw Exception
      \EndIf
    \EndFor
  \EndFor
  \State \Return $\Tile$
  \end{algorithmic}
\end{algorithm}  

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> alg-tiler.tex <==
\begin{algorithm}[!t]
  \caption{\ourtool($\PP, \Psi_{pre}, \Psi_{post}$)}
  \label{alg:tmc}
  \begin{algorithmic}[1]
    \Require $\PP, \Psi_{pre}, \Psi_{post}$
    \Ensure Output Success or Fail
    \State $\Tile$ := TileGen($\PP, \alpha, \beta$);
    \State $\ppost$ := GenMidConds($\PP, \Psi_{pre}, \Psi_{post}, \Tile$);
    \State $res = TRUE; proved = FALSE$
    \For {each loop $\LL_n = for(k:=\EE;\mexit{\LL};k:=\EE) ~\{~ \LB ~\} \in \mathcal{L}$}
      \While {$proved = FALSE$}
        \State $res := res \wedge$ TMC($\LL_n, \ppost_{\LL_{n-1}}, \ppost_{\LL_n}$)
        \If{$res = TRUE \vee |\ppost_{\LL_n}| \neq 0$}
          \State $proved := TRUE$
        \Else
          \State $proved := FALSE$
          \State $\ppost_{\LL_n}$ := Refute($\LL,\ppost_{\LL_{n-1}},\ppost_{\LL_n}$)
        \EndIf
      \EndWhile
      \State $proved = FALSE$
    \EndFor
    \If {$res == TRUE$}
      \Return Verification Successful
    \Else
      \Return Verification Failed
    \EndIf
  \end{algorithmic}
\end{algorithm}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> alg-tiling.tex <==
\begin{algorithm}[!t]
 \caption{\textsc{OurAlg}()}
 \label{alg:tiling}
\begin{algorithmic}[1]
  \Require $P$ with a single loop and an assertion $\formula = \forall j.\; (lb' \leq j <  ub' \limplies good'( a[j]) )$ after the loop
  \Ensure A loop invariant that proves the assertion
  \State $\program',i,j,good := \textsc{Instrument}(\program,\formula)$
  \State $I := \textsc{InvGen}(\program')$\hfill//may need iterative calls
  if some assertions fail
  \State $\tile(i,j) := \textsc{GetTile}(I,i,j)$
  \State $ub(i) := \textsc{getUpperBoundExpression}(\tile,i,j)$
  \State $lb(i) := \textsc{getLowerBoundExpression}(\tile,i,j)$
  \State Check the following formulas are unsat
  \State $\tile(k,j') \land \tile(k+1,j'') \land j' < j < j'' \land \lnot \tile(k,j) \land \lnot \tile(k+1,j)$ \hfill {//compact}
  \State $j' < j < j'' \land \tile(k,j') \land \tile(k,j'') \land \lnot \tile(k,j)$  \hfill {//range like}
  \State $k \neq k' \land \tile(k,j) \land \tile(k',j)$ \hfill {//disjoint}
  \State $I(x) \land \tile(i,j') \land (\Lor_{p \in paths}\; \Land_{j \in \text{array accesses in } p} j' \neq j)$ \hfill {//all access in tiles}
  \State if all the above checks succeed then we have proven the following invariant
  \State $\forall j.\; (lb(0) \leq j < ub(i) \limplies good( a[j]) )$
  \If{$\forall x.\; lb(0) \leq lb' \land (loopExitCondition \land I \limplies ub' \leq ub(i) ) \land good \limplies good'$}
  % \If{$\exists e. (loopExitCondition \limplies e = i) \land  \forall j.\; (lb(0) \leq j < ub(e) \limplies good( a[j]) ) \limplies \formula$}
  \EndIf
  \State \Return{$\forall j.\; (lb(0) \leq j < ub(i) \limplies good( a[j]) )$} 
\end{algorithmic}
\hrule
\paragraph{More on our example:}
Get the following invariant from Invgen like tools for the second loop.
$$
\tile = 4i-4 \leq j <  4i
$$
$j$ is a variable that non-deterministically takes values of indexes
that were written in an iteration.

$I$ suggests that good values are written the loop in the tiles of 4.
We need to check the following two things about the tiles
\begin{itemize}
\item tiles are disjoint across iterations
\item tiles are range-like
\item tiles are compact, i.e., there is no gap between the tiles
\item Each index in a tile is accessed during the corresponding iteration
\end{itemize}
\vspace{\jot}
\end{algorithm}  

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> alg-tmc.tex <==
\begin{algorithm}[!t]
  \caption{TMC($\LL, \Tile, \Psi_{pre}, \Psi_{post}$)}
  \label{alg:tmc}
  \begin{algorithmic}[1]
%    \Require $P:=\psi^l_{pre}; Loop ~ l; \psi^l_{post}$, Tiles $\tile_a$
    \Require $\LL= for(k:=\EE;\mexit{\LL};k:=\EE) ~\{~ \LB ~\} \in \mathcal{L}, \Tile, \Psi_{pre} = (\forall k_1,k_2, ... \phi_{pre}(k_1, k_2, ...) \rightarrow \psi_{pre}(\A_1[k_1],\A_2[k_2], ...)), \Psi_{post} = (\forall k_1,k_2, ... \phi_{post}(k_1, k_2, ...) \rightarrow \psi_{post}(\A_1[k_1],\A_2[k_2], ...))$
%TODO Need to add other program variables in \psi_{post}.
    \Ensure Output Success or Fail
    \State Create $\LL'= for(k:=\EE;\mexit{\LL};k:=\EE) ~\{~ \LB' ~\}$ where $\LB'$ consists of following stmts
    \State \mbox{}\hspace{5ex} `$i=*;$'
    \State \mbox{}\hspace{5ex} \textbf{for} each array $\A_n \in \mathcal{A}$ \textbf{do}
    \State \mbox{}\hspace{10ex} `$j_{\A_n}=*;$'
    \State \mbox{}\hspace{5ex} `assume($i \geq \alpha_{\LL} \land Cond_{\LL}$);'
    \State \mbox{}\hspace{5ex} `assume($\Psi_{pre}$);'
    \State \mbox{}\hspace{5ex} \textbf{for} each array $\A_n \in \mathcal{A}$ \textbf{do}
    \State \mbox{}\hspace{10ex} `assume($\Tile_{\LL,\A_n}(i,j_{\A_n})$);'
    \State \mbox{}\hspace{5ex} `$\LB$;'
    \State \mbox{}\hspace{5ex} $\Psi$ = $\Psi_{post}$
    \State \mbox{}\hspace{5ex} \textbf{for} each array $\A_n \in \mathcal{A}$ \textbf{do}
    \State \mbox{}\hspace{10ex} $\Psi$ = $\Psi[j_{\A_n}/k_n]$);
    \State \mbox{}\hspace{5ex} `assert($\Psi$);'
    \State \Return BMC($\LL'$)
  \end{algorithmic}
\end{algorithm}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> algorithms.tex <==
%\subsubsection{Verification using Tiles}

In this subsection, we describe the algorithms used 
for tiling the array indices and use them
to verify the given assertion.

\subsubsection{Tile Generation}
Refer to the \textit{tile} generation algorithm \ref{alg:tilegen}.
%Let $e^a_n$ be $n^{th}$ index expression for the array $a$
%over loop counter $i$ in loop $l$.
%We use \clang~ to extract the expressions used as an index
%to an array in the current loop and
%\cbmc~ to check if the loop counter $i$ is modified in the loop body.
%If the loop counter $i$ is not modified in $l$'s body then the
%index expressions $e^a_n$ are use to compute the 
%lower bound $lb=\forall n. min(e^a_n)$ and the upper bound
%$ub=\forall n. max(e^a_n)$. 
%To get a lower bound $lb$ we use the semantic equivalence
%$lb = \forall n. min(e_n)
%\simeq
%\bigwedge\limits_{k=1}^n (lb \leq e_n) \land \bigvee\limits_{k=1}^n (lb \geq e_n)$.
%A similar equivalence gives the upper bound.
%$lb \leq i \leq ub$ is assumed as the \textit{tile}
%for array $a$ in that loop $l$.

Formula $\phi_d$ represents \textit{Disjointness}, 
%$\phi_r$ represents \textit{Rangelike},
$\phi_c$ represents \textit{Compactness} and
formulas $\phi_{lb}$ and $\phi_{ub}$ represent \textit{Inclusion of Boundaries}.
If $\phi_d$ is \textit{unsat},
no index value occurs in two different \textit{tiles}.
If $\phi_c$ is \textit{unsat},
there are no gaps between any two consecutive \textit{tiles}.
%If $\phi_r$ is \textit{unsat},
%there are no indices within a \textit{tile} that is missed.
If $\phi_{lb} \land \phi_{lb}$ is \textit{sat},
boundary indices are included in the analysis.
%These checks ensure that entire range of 
%array indices is covered by the \textit{tile}.

\input{alg-tilegen}

\input{alg-tmc}

\input{alg-tiler}

Once a valid \textit{tile} is obtained for a loop $l$,
we need to check if given a pre-condition to the loop $l$,
the post-condition holds.
This is equivalent to checking if the post-condition
holds at all the indices in the \textit{tile}.
We call this \textbf{Tiled Model Checking(TMC)} and is described in
algorithm \ref{alg:tmc}.
We assign a non-deterministic value to the loop counter $i$ and
a introduce new loop counter $j$.
We restrict the value of the loop counter $i$ using its initialization
in the loop $l$ and the loops exit criterion.
We then assume the pre-condition for the loop $l$.
We assume that $j$ takes values from the \textit{tile} 
for all arrays read or written to in loop $l$.
We then put the loop body for $l$.
Finally, we assert the post-condition of the loop $l$ where
new loop counter $j$ which takes values from the \textit{tile}
is substituted for $i$.
Thus, the assertion is checked at only the indices
present in the \textit{tile}.
If $l$ is the last loop then the post-condition
is the assertion given in the input program where all the array elements
are accessed linearly.
We use \clang~ as the front end to extract the loop body
as well as inserting assume and assert statements and
to perform the substitution operation.
We then execute the bounded model checker \cbmc~ to get
the verification result.

\textbf{Refine} Refuted post-conditions reported by \cbmc 
are removed in the subsequent iteration.
The refinement loop iterates till either all post-conditions are proven
or there are none left, which implies that the pre-condition for the
next sequentially composed loop is ``true''.
Once post-conditions are proven, the tool proceeds
to the next sequentially composed loop.
\ourtool reports success when the final assertion in the code is
proven.


==> discuss.tex <==
\section{Limitations of Existing Tools}
Booster \cite{booster}, an acceleration-based verification tool for array programs, runs indefinitely on the program shown in Figure \ref{prog:motex}. This happens because it is unable to reason that all the array entries are updated and the update is with values that do not violate the assertion. For our program it is not the case that some array entries still contain the DEFAULTVALUE, and may violate the assertion $\phi$. \\

Reasoning about indices needs an analysis that under-approximates, since the invariants over indices form the guards in the quantified array invariants, for example $0 \leq i \leq k \Rightarrow a[i] = 0$. Available invariant generation tools, however, over-approximate when discovering invariants, limiting the usage of such tools for generating invariants over array indices.

\section{Invariant Generation using InvGen}
The modified program shown in Figure \ref{prog:proginvgen} is given as input to InvGen \cite{invgen} for generating invariants over the array index. The modifications included removing the arrays from the program(since they are not handled by InvGen), introducing auxiliary variables $j_1, j_2, j_3, j_4$ and $j$ to store the value of the array index expression at different points in the program and putting a assertion over the indices updated in-place of the original quantified assertion over the array. InvGen generates the invariant $\mathcal{I} = (j_1 - \frac{1}{4}j - 3i \leq -3 \wedge j_1 - j >= 0 \wedge j_1 - 3*i >= -3)$ for this program. On eliminating $j_1$, we have $\mathcal{I} = (0 \leq j \leq 4*i - 4)$. This invariant $\mathcal{I}$ is an over-approximation of the state-space at the head of the loop.

\begin{figure}
\begin{minipage}[b]{0.5\textwidth}
\begin{verbatim}
int main()
{
 int DEFAULTVALUE=1, MINVAL=2;
 int CCCELVOL4 = 5;
 int CCCELVOL3 = 7;
 int CCCELVOL2 = 3;
 int CCCELVOL1 = 1;
 int CELLCOUNT, i, j=0;
 int j1=0, j2=0, j3=0, j4=0;
 int NONDET;

 for(i=1; i<=CELLCOUNT/4; i++)
 {
  j1=-1; j2=-1; j3=-1; j4=-1;
  if(CCCELVOL4 >= MINVAL)
  {
  	j4 = i*4 - 4;
  }
  else
  {
  	j4 = i*4 - 4;
  }

  if(CCCELVOL3 >= MINVAL)
  {
  	j3 = i*4 - 3;
  }
  else
  {
  	j3 = i*4 - 3;
  }

\end{verbatim}
\end{minipage}
{\vrule}
\begin{minipage}[b]{0.5\textwidth}
\begin{verbatim}
  if(CCCELVOL2 >= MINVAL)
  {
  	j2 = i*4 - 2;
  }
  else
  {
  	j2 = i*4 - 2;
  }

  if(CCCELVOL1 >= MINVAL)
  {
  	j1 = i*4 - 1;
  }
  else
  {
  	j1 = i*4 - 1;
  }
  
  if(NONDET) {
    j = j4;
  } else if (NONDET) {
    j = j3;
  } else if (NONDET) {
    j = j2;
  } else {
    j = j1;
  }
 }

 assert(0 <= j && j <= CELLCOUNT);
 return 0;
}
\end{verbatim}
\end{minipage}
\label{prog:proginvgen}
\caption{Program input to InvGen}
\end{figure}

\section{Proving the Assertion}
\subsection{Interpretation of the Invariant}
We introduce two predicates that relate the values that array elements can take on and if a particular array location was written. The predicate $good(a[k])$, for some index $k$, is true if $a[k]$ takes a value that does not violate the assertion and is false otherwise. In our example, $good(volArray[k]) = volArray[k] \geq MINVAL || volArray[k] = 0$. The predicate $written(a[j],i)$ is true if $a[j]$ was updated with some value in the $i^{th}$ iteration of the loop. \\

The assertion at the end of the loop is $\phi = \forall k (0 \leq k < CELLCOUNT) \Rightarrow good(a[k])$. \\

The invariant needed to prove the assertion is $\mathcal{I'} = \forall i \forall j. (0 \leq j \leq 4*i-4) \Rightarrow good(a[j])$, where $i$ is the loop iterator. $(\mathcal{I'} \wedge \neg (i \leq CELLCOUNT/4)) \Rightarrow \phi$.\\

The invariant given by InvGen can be interpreted as $\mathcal{I} = \forall i \forall j. written(a[j],i) \Rightarrow ((0 \leq j \leq 4*i-4) \wedge good(a[j]))$ where $i$ is the loop iterator and $j$ represents the values of the array index expressions in the current iteration. It says that if an array index was updated (i.e. written(a[j],i)) then it takes a good value and the range of the array index expression is between $0$ and $4*i-4$. This invariant is not strong enough to prove the assertion. $(\mathcal{I} \wedge \neg (i \leq CELLCOUNT/4)) \not\Rightarrow \phi$.

\subsection{Problem}
One of the reasons why this invariant is unable to prove the assertion is that it is \textit{not tight}. $j$ may not take all the values $0 \leq j \leq 4*i-4$ as specified in the invariant $\mathcal{I}$, hence it may \textit{not be tight}. Inorder to be able to prove the assertion, we need to show that all the array entries have been updated, which in turn amounts to showing that $j$ actually does take all the values in the specified range at the loop head for the program in Figure \ref{prog:proginvgen}. Formally, $\Gamma = \forall i \forall j. (4*i - 4 < j \leq 4*i) \Rightarrow written(a[j],i)$. \\

In general, we need to infer a formula $\Gamma$ such that the following conditions hold:
\begin{enumerate}
\item $\mathcal{I} \wedge \Gamma \Rightarrow \phi$\\
This condition says that $\Gamma$ should be able to tighten the loop invariant so that the assertion can be proven. This condition also says that $\Gamma$ is related to $\mathcal{I}$, because in conjunction with $\mathcal{I}$ it proves the assertion.
\item $\mathcal{I} \wedge \Gamma \rightarrow_{body} \Gamma$\\
On a single iteration though the loop body, $\Gamma$ should hold. In other words, $\mathcal{I} \wedge \Gamma$ is a loop invariant. We need not check the condition $\mathcal{I} \wedge \Gamma \rightarrow_{body} \mathcal{I}$, since we already know that $\mathcal{I}$ is a loop invariant.
\end{enumerate}

We call a formula $\Gamma$ that satisfies the above conditions a \textit{difference invariant}. Note that $\Gamma$ is a conditional loop invariant. $\Gamma$ on its own may not be a loop invariant. However, we need to ensure that given $\mathcal{I}$ is a loop invariant, $\mathcal{I} \wedge \Gamma$ is a loop invariant, a stronger one.

\subsection{Comparison with Abduction}
Suppose we want to abduct the reason for the implication $\phi_1 \Rightarrow \phi_2$ to hold. Abduction tries to infers formulas $\phi_3$ such that if $\phi_3$ holds for all the executions of the program then $\phi_1 \wedge \phi_3 \Rightarrow \phi_2$ holds. Abduction is for arbitrary formulas. The inference of $\phi_3$ is independent of the loop body. Also it does not ensure loop invariance of the conjunction $\phi_1 \wedge \phi_3$. Thus, the obtaining a \textit{difference invariant} is not the same as abduction.

\subsection{Inferring $\Gamma$ from Counterexamples}
Consider the counterexample trace obtained from a analysis tool. Since $\mathcal{I}$ is a loop invariant, the counterexample satisfies $\mathcal{I}$. If we run the concrete counterexample on the program, we figure that the counterexample does not violate $\phi$ ($\because \phi$ holds for the program). Hence we can conclude that the trace is spurious. At this point we are interested in asking why is the counterexample trace unable to reach the states the satisfy $\mathcal{I}$ but do not satisfy $\phi$. The answer to this question is the additional property $\Gamma$ that holds for all spurious counterexamples but is not captured by the loop invariant $\mathcal{I}$.

\subsection{Characterization of $\Gamma$}
A two step approach is visualized, where in the first step from the program, assertion, the loop invariant and the reported counterexamples a guess is made of the \textit{category} from which property that will be needed to prove the assertion. The property ``Every array index is updated'' is an example of a category. One of the heuristic, for example, compares the spurious trace with the corresponding concrete trace. The differences in the program values in concrete and abstract trace provide a valuable insight for fixing the \textit{template}. \\

Once the template is decided, it is then instantiated with the program variables. The instantiation is checked for satisfaction of the two conditions for difference invariants. If it does not satisfy the first condition, then we know that we need to tighten the inference $\Gamma$. If it does not satisfy the second condition then it means that the inference $\Gamma$ under the invariance of $\mathcal{I}$ is not a loop invariant. Hence, will not be interested in such formulas.

\section{Viewpoints on Difference Invariant}
The invariant given by InvGen for the program in Figure \ref{prog:proginvgen} is $\mathcal{I} = (0 \leq j \leq 4*i - 4)$. Suppose that after a fixed number of iterations $k$, the states observed are given by constraint $(0 \leq j \leq 4*k - 4)$. After executing one more iteration of the loop (i.e. $(k+1)^{st}$ iteration), we can see that the variable $j$ takes on the new values given by the constraint $4*k - 4 < j \leq 4*k$. This constraint describes the new states that the variable $j$ will see if we take the $(k+1)^{st}$ iteration of the loop. We call such a constraint a \textit{Difference Invariant}. Clearly, the loop invariant is independent of the iteration count, whereas the \textit{difference invariant} is dependent on the iteration count as well as on values of other program variables, such as variable $i$ in our program, in the $(k+1)^{st}$ iteration of the loop. \\

The loop invariant can be viewed as (possibly infinite) union of a \textit{generic tile}(constraint) representing states observed during a loop iteration. Abstract interpretation makes it possible to compute this union in finite way by using join and widening operators. Note that the tile generated by the widening operator is, usually, not a \textit{generic tile}. The \textit{difference invariant} can be thought of as a \textit{generic tile} of the loop invariant. Inorder to prove that a loop invariant is \textit{tight}, it suffices to prove, assuming that $j$ takes all the values till the $i^{th}$ iteration, in the $(k+1)^{st}$ iteration $j$ takes all the values given by the \textit{generic tile} of the loop invariant (i.e. the \textit{difference invariant} corresponding to the $(k+1)^{st}$ iteration). \\

\textit{Tiling} a given loop invariant is not easy. One of the problems is that if the loop invariant represents an open region in the $n$-dimensional space then observing the new states that got added to the loop invariant by executing one more iteration of the loop becomes hard. For our example, the invariant $\mathcal{I}$ represents a open region, since the loop iteration counter $i$ is not constrained. \\

\textit{An attempt:}\\
Let $k$ represent a symbolic bound on the value of $i$. Thus, we add the constraint $i \leq k$ to our invariant which is given as $\mathcal{I}=(0\leq j \leq 4*i - 4) \wedge (i \leq k)$. The invariant after one more iteration of the loop is given by $\mathcal{I'}=(0\leq j \leq 4*i - 4) \wedge (i \leq k+1)$. We are tempted to assume that $\mathcal{I'} \wedge \neg \mathcal{I}$ will be the \textit{difference invariant}. The simplification is given below:

\begin{align*}
& \mathcal{I'} \wedge \neg \mathcal{I} \\
& \equiv ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1)) \wedge \neg ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k)) \\
& \equiv ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1)) \wedge ((0 > j) \vee (j > 4*i - 4) \vee (i > k)) \\
& \equiv ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1) \wedge (0 > j)) \\ &\ \ \vee ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1) \wedge (j > 4*i - 4)) \\ &\ \  \vee ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1) \wedge (i > k)) \\
& \equiv ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i \leq k+1) \wedge (i > k)) \\
& \equiv ((0\leq j) \wedge (j \leq 4*i - 4) \wedge (i = k+1)) \\
& \Rightarrow ((0\leq j \leq 4*k))
\end{align*}

This does not seem to give the desired constraint $(4*k - 4 < j \leq 4*k)$. \\

Let the unprimed variable names indicate the value of the variable before executing the loop body (e.g. variable $i$) and the primed variable names indicate the value of the variable after the loop body (e.g. variable $i'$). We will denote the \textit{difference invariant} by $Diff(y,\alpha)$, where $y$ is a vector of program variables, $y$ contains unprimed variables at the beginning of the loop and contains primed variables at the end of the loop, and $\alpha$ is a vector of auxiliary variables used to store the values of array index expressions. Different auxiliary variables are used for storing the values of different expressions at different program points. Hence, auxiliary variables are assigned only once. 

\section{Possible Solutions}
\subsection{A naive approach}
The loop body can update a variable with different values only a small number of times. The range of values, as given by the \textit{difference invariant}, that needs to be checked will be finite and small. With multiple calls to CBMC\cite{cbmc}, it can be checked if the variable $j$ is assigned each of the values in this range. For example, to check if $j$ takes the value $4*i - 3$, we put the assert statement $assert(j \neq 4*i - 3);$ to which CBMC finds a counterexample. This means that $j$ takes the value $4*i - 3$ along some run. Repeating the similar process for other values, we can check if $j$ takes all the values in the range.

\subsection{Translation to SMT}
\subsubsection{Using Diff at the end of the loop iteration}
Let the pre-condition on a vector of variables $x$ at the beginning of the loop be represented by $Pre(x)$. Let the transition formula $T(x,x')$ denote the updation of the variables by the loop body. Given that $Pre(x)$ is the pre-condition after $k$ iterations of the loop, let $Diff(x',\alpha)$ represent the \textit{difference invariant} after executing the $(k+1)^{st}$ loop iteration.

The \textit{tightness} check corresponds to the following SMT formula, for all states $x'$ in the difference there is some state $x$ in $Pre$ that reaches this state after taking the transition $T(x,x')$. If this formula is true then the invariant is tight.

\[
\forall x',\alpha. (Diff(x',\alpha) \rightarrow (\exists x. (Pre(x) \wedge T(x,x') ))) 
\]

Notice that for all the $\alpha$'s in the \textit{difference invariant}, the formula need to find a state $x$ in $Pre$ that reaches a state $x'$ such that the value of one of the array access is $\alpha$ along that execution. 

The negation of this formula asks does there exists some value $x'$ that satisfies $Diff(x')$ such that no matter what value of $x$ is taken to begin with that satisfies $Pre(z)$, we cannot reach the value $x'$ upon taking any transition $T(x,x')$. The invariant is tight if this formula is \textit{unsat}. If this formula has a satisfying assignment then the loop invariant is not tight.

\[
\exists x', \alpha. (Diff(x',\alpha) \wedge (\forall x. (Pre(x) \rightarrow \neg T(x,x') )))
\]

\subsubsection{Using Diff at the beginning of the loop iteration}
Given that $Pre(x)$ is the pre-condition after $k$ iterations of the loop, let $Diff(x,\alpha)$ represent the \textit{difference invariant} guessed for the $(k+1)^{st}$ loop iteration. We specify a stronger \textit{tightness} check: for all states $x$ in the $Pre(x)$, for all the values $\alpha$ of the auxiliary variables that satisfy the  \textit{difference invariant}, along all the paths through the loop (if the program is deterministic then there is only one path) one of the array access expressions is equal to $\alpha$.

\[
\forall x,\alpha. \; Pre(x) \land Diff(x,\alpha) \limplies
\Land_{p \in paths}\quad \Lor_{j \in \text{array accesses in } p} \alpha = j
\]

\textit{Advantages:}
\begin{itemize}
\item The formula does not involve a quantifier alternation and hence is more amenable to existing SMT solvers
\item Easy to observe association between the vector $x$ in $Pre$ and a auxiliary variables $\alpha$ that satisfy $Diff$
\item Needs all the states $x$ in $Pre$ associated with $\alpha$ to have a valid path where a array access expression takes the values $\alpha$
\end{itemize}

\input{alg-tiling}
\input{alg-instrument}

%\ashu{formula}

% \begin{itemize}
% \item For all iterations
% \item if we start from a state in pre then
% \item all executions from the state along the body
% \item accesses all the arrey indexes in the array block corresponding to the
% iteration
% \end{itemize}

%\begin{itemize}
%\item if we start from a state in pre then
%\item all the executions from the state along the body
%\item accesses all the arrey indexes {\em that satisfy Diff}
%\end{itemize}
%$$
%\forall x,\alpha. \; Pre(x) \land Diff(x,\alpha) \limplies
%\Land_{p \in paths}\quad \Lor_{j \in \text{array accesses in } p} \alpha = j
%$$

%Constraints for reachability of some iterations, tiling parameters,


%\divesh{ formula}

%\begin{itemize}
%\item For all iterations of the loop
%\item there exists a state in pre such that
%\item forall array index accesses in the array block corresponding to the
%iteration
%\item there exists a executions from the state along the body
%\end{itemize}

\section{Impediments to Implementation}
The following aspects act as impediments to a fully automated tool:

\begin{enumerate}
\item \textit{Instrumentation for Invariant Generation} \\
InvGen did not scale for generating invariants after applying the instrumentation procedure  \label{alg:tiling} described above. The following changes were made for the instrumentation to work:
\begin{itemize}
\item $j := UNINIT$ moved from end of body to begin of body.
\item Non-det if-else ladder for updating $j$ removed. The value of $j$ is now updated non-deterministically with the array index expression when a array element is updated.
\item $assume(j != -1); assert(j != jold);$ introduced in place of $assert(j\_old \neq  UNINIT \land j \neq  UNINIT \limplies j\_old \neq j);$
\item Assertion on the values written to array elements removed for scalability; may need a separate pass.
\end{itemize}
With these changes after instrumentation scales for the ``periodic'' class of programs except ``periodic-range5.c'' where is takes more than an hour. Need to explore ways of instrumentation that can improve the performance and scalability of InvGen for invariant generation.

\item \textit{Lower bound of the invariants generated using InvGen} \\
Since $j$ is initialized to $UINIT$ at the beginning of the loop and in subsequent iterations, the lower bound of the generated invariant is $UINIT$. This also affects the tile extraction using quantifier elimination.

\item \textit{Extraction of Tiles from Invariants} \\
Quantifier elimination cleans the invariant generated from InvGen of the auxiliary variables. The resultant invariant is not necessarily in the form of a tile. Heuristics for tile extractions are to be devised and implemented.

\item \textit{Automation of the checks for a tile} \\
Need to figure out the Z3 apis for transformation of the formula generated after quantifier elimination for checking compactness, rangelike and disjointedness constraints.

\item \textit{CBMC for checking ``All access in tile''} \\
$j' = nondet();$ \\
$assume I(x) \wedge \tau(i,j');$ \\
$flag = false;$\\
transformed loop body with $if(j==j') flag = true;$ inserted after each update to $j$ \\
$assert(flag == true);$ \\ \newline

If the assertion is false then there is an index in $\tau$ that is not updated in the array. Need to verify if this strategy will work. Do we need I(x)? 

Extracting the loop body from the source program for which we are checking the property will need some attention. Currently extracting the body of the second loop in the program.

\end{enumerate}


\section{Compositionality and Pre-conditions}
The algorithm \ref{alg:tiling} does not handle a sequential composition of the loops. Primary reason is that the algorithm does not produce any pre/post-conditions; it only concludes if the given assertion holds or not. In order to make the given technique compositional, a proposed method is to compute a pre-condition which is necessary for the assertion to hold after the given loop. In general, this is a hard problem. To circumvent this, we assume that a static analysis or an oracle gives this precondition before the loop. The analysis now need to take into consideration the effect of this precondition before concluding the validity of the given assertion. Thus, the updated problem definition is given a precondition before the loop, a single program loop and an assertion at the end of the loop, decide if the assertion holds. \\

\textit{Incorporating the precondition in the analysis}:\\
The effect of precondition needs to be taken into account in two things 1) generation of tile and 2) verifying if the assertion holds for all accesses in the tile, given the precondition. \\

The generation of tiles should take into account the given precondition and generate the tiles such that the compositionality is not violated.  This will ensure that the tileness checks such as compositionality, range-like and disjointness are not impacted by the presence of the precondition. Consider the example shown in figure \ref{fig:multiloop} for concreteness. The tile generator should generate the tile $(2*i-2 \leq j \leq 2*i-1)$ even if only index 2*i-1 is accessed in the loop due to the presence of the precondition. \\

\begin{figure}[h]
{\scriptsize
\begin{verbatim}
for(i = 1; i <= COUNT/2; i++)
{
 if(CCCELVOL2 >= MINVAL)
 {
   a[i*2 - 2] = 2;
 }
 else
 {
   a[i*2 - 2] = 0;
 }
}
//\forall i; (1 <= i <= COUNT/2 \implies a[i*2 - 2] = 2)
for(i = 1; i <= COUNT/2; i++)
{
 if(CCCELVOL1 >= MINVAL)
 {
   a[i*2 - 1] = 1;
 }
 else
 {
   a[i*2 - 1] = 0;
 }
}
for(i = 0; i < COUNT; i++)
{
 assert(a[i] >= MINVAL || a[i] == 0 );
}
\end{verbatim}
}
\label{fig:multiloop}
\end{figure}

Verifying if the assertion holds at all the access indices in the tile in presence of the precondition amounts to assuming an appropriate condition at the beginning of the loop body. For the example shown in figure \ref{fig:multiloop}, the precondition for the second loop is given as \textit{assume(a[i*2 - 2] = 2)}. \\

\textit{A point of concern}:\\

\begin{figure}[h]
{\scriptsize
\begin{verbatim}
for(i = 1; i <= COUNT/3; i++)
{
   a[i*3 - 3] = 3;
}
//\forall i; (1 <= i <= COUNT/3 \implies a[i*3 - 3] = 3)
for(i = 1; i <= COUNT/2; i++)
{
   a[i*2 - 2] = 2;
}
\end{verbatim}
}
\label{fig:tilesize}
\end{figure}

In the example shown in the figure \ref{fig:multiloop}, all the loops had the same tile size. However, it may not be the case for program in general. Consider the loops shown in the figure \ref{fig:tilesize}. The first and the second loop have the different tile sizes. We propose to take the LCM of both the tile sizes as the tile size for both the loops. While performing the all access in tiles check, we need to unroll the first loop twice and the second loop thrice for soundness. \\

\textit{Aggregation in precondition}:\\
\begin{figure}[h]
{\scriptsize
\begin{verbatim}
// assume size = 100 * total;
for(i=0;i<total;i++)
{
 wtSum = wtSum + weight[i];
}
//Midcondition: wtSum = \Sigma_i weight[i]
if(wtSum<=size)
{
 k=0;
 for(i=0;i<total;i++)
 {
  numIns = weight[i];
  for(j=0;j<numIns;j++) 
  {
   assert(k < 100 * total);
   arr[k++] = i;
  }
 }
}
\end{verbatim}
}
\label{fig:midcond}
\end{figure}

Consider the example shown in the figure \ref{fig:midcond}. The mid condition is not quantified but has an aggregation function. It is not exactly clear as to how to incorporate the effect of this preconditon. \\


\textit{Discussion with Supratik} \\

Consider the example shown in the figure \ref{fig:inc-pre}. The pre-condition says that the entire array is initialized to value 1. The first loop accesses every third element and writes the value 3 to the array. Thus the array contents have the pattern 3 1 1 3 1 1 so on. The post-condition of this loop is $\forall i. (1 \leq i \leq COUNT/3 \implies (a[i*3 - 3] = 3 \wedge a[i*3 - 2] = 1 \wedge a[i*3 - 2] = 1) )$. This becomes the pre-condition for the second loop. The second loop accesses every second element in the array and multiplies it by two. Thus the array contents have the pattern 6 1 2 3 2 1 6 1 2 3 2 1 so on. We would like to verify that every sixth entry in the array has the value 6. \\

\begin{figure}[h]
{\scriptsize
\begin{verbatim}
//PC: \forall i; (1 <= i < COUNT \implies a[i] = 1)

for(i = 1; i <= COUNT/3; i++)
{
   a[i*3 - 3] = 3;
}

//MC:\forall i; (1 <= i <= COUNT/3 \implies (a[i*3 - 3] = 3 \wedge 
a[i*3 - 2] = 1 \wedge a[i*3 - 1] = 1) )

for(i = 1; i <= COUNT/2; i++)
{
   a[i*2 - 2] = a[i*2 - 2] * 2;
}

//ASSERTION:\forall i; (1 <= i <= COUNT/6 \implies (a[i*6 - 6] = 6))
\end{verbatim}
}
\label{fig:inc-pre}
\caption{Incorporating pre-conditions}
\end{figure}

Mapping the indices from the mid-condition to the indices being accessed in the body is difficult and hinders the exchange of information between the loops. We thus assume that the pre-conditions/mid-condition can be represented in a standard normal form described as $\forall i. (0 \leq i < length(array) \implies \phi_i )$. The formula $\phi_i$ describes the property of the $i$ element of the array. We use an existentially quantified variable to get the formula $\phi_i$ from the original mid-condition. Consider the midcondition for the example \ref{fig:inc-pre}. The normalized form is given as $\forall i. (0 \leq i < COUNT \implies (\exists j. (1 \leq j \leq COUNT/3) \wedge (i=j*3 - 3 \implies a[i] = 3) \wedge (i=j*3 - 2 \implies a[i] = 1) \wedge (i=j*3 - 1 \implies a[i] = 1) )$.\\

The normalized form can be easily modelled for the CBMC check. We introduce a new nondet variable $j$ and put an assume on its value allowing it to access a specified range; $(1 \leq j \leq COUNT/3)$ is the range for our example. The formula $\phi_i$ then becomes the part of the loop body and $i$ is replaced with the index expression accessed in the loop. A similar transformation applies for the given assertion. The following code demonstrates this transformation for the second loop of example \ref{fig:inc-pre}: \\

\begin{figure}[h]
{\scriptsize
\begin{verbatim}
   i = nondet();
   assume(1 <= i && i <= COUNT/2);
   j = nondet();
   assume(1 <= j && j <= COUNT/3);
   
   if(i*2-2 == j*3-3) assume(a[i*2-2]==3);
   else if(i*2-2 == j*3-2) assume(a[i*2-2]==1);
   else if(i*2-2 == j*3-1) assume(a[i*2-2]==1);
   
   a[i*2-2] = a[i*2-2] * 2;
   
   k = nondet();
   assume(1 <= k && k <= COUNT/6);
   if(i*2-2 == k*6-6) assert(a[i*2-2]==6);
\end{verbatim}
}
\label{fig:cbmc-modeling}
\caption{Modelling for CBMC}
\end{figure}

We have essentially made two assumptions:
\begin{itemize}
\item The normalized mid-condition specifies a property on all the array indices
\item Each array index maps to exactly one pair consisting of a tile and an index in that tile
\end{itemize}

While the first condition helps us avoid the dependence on having the same tile size across loops, the second condition makes sure that the mapping from one form of tilling to another form of tilling can be done consistently.

\section{Generating Mid-conditions}

The following algorithm describes mid-condition generation using Daikon.

\begin{algorithm}[!t]
 \caption{\textsc{Instrumentation for Invoking Daikon}}
 \label{alg:instdaikon}
\begin{algorithmic}[1]
  \Require Program $P$ with arrays of same $size$, non-nested loops and a main, the set of tile structures ${\tile_a}$ for each array $a \in P$, the set $Vars$ of non-constant scalar variables
  \State Initialize all arrays in main with random values
  \ForAll{$a \in P$}
%    \Comment{Initialize all arrays in main}
    \State Output - for($i=0; i < size; i++$) { $a[i] = rand();$ } 
  \EndFor
  \State Create a map $map$ between string representations of $a[iExpr]$ and scalar variable representing it
    \ForAll{$a \in P$}
      \ForAll{$\tile^k_a \in {\tile_a}$}
        \ForAll{$iExpr \in \tile^k_a$}
          \State create new scalarVar name
          \State map[string(scalarVar)]=string($a[iExpr]$)
        \EndFor
      \EndFor
    \EndFor

  \State Add dummy function calls at the end of body in all loops
  \ForAll{loops $l \in P$}
    \State Output - Loop\_l(
    \ForAll{$key \in map$}
      \State Output $map[key]$,
    \EndFor
    \ForAll{$v \in Vars$}
      \State Output $v$,
    \EndFor
    \State Output - iterator $i$ of $l$);
  \EndFor

  \State Create empty definitions for introduced dummy functions
  
\end{algorithmic}
\end{algorithm}


\section{Ideas moving forward}

The current set of constraints on the tile are too restrictive and 
in some sense do not really use the property at hand.
We need to investigate the find the necessary condition for a tile
such that the soundness proof goes through.
Such so called ``necessary conditions'' may not be automatically
checkable, however, they guide us towards the relaxation of these
constraints that are needed to automate the check for these constraints.
Consider the disjointness check, it is a strong constraint which
says that the indices to which the updates are made do not overlap. 
What is essentially needed for the proof to go through is a 
non-interference condition which says that the updates made are 
such that they do not destroy the truth value of already 
established slices of the desired property. 
For example, consider an example that updates entries in an array 
``a'' at locations ``i'' and ``i-10'' where the property says that 
the difference ``a[i-10] - a[i]'' is some constant. 
If we consider {i,i-10} as the tile, clearly it is not disjoint.
However, non-interference can be established for the given property.

Another important point is that we do not want to restrict what 
we call a tile by giving it a definition. 
We want to define the constraints and any thing that satisfies 
these constraints is a tile.

\subsection{Exploring tile generation}
The current approach for tile generation is kind of a 
guess-and-check approach.
Explore if we can pose the problem of tile generation 
as a optimization problem.
If we can specify the tileness conditions as a system
of constraints say using Horn Clauses then we can feed them to
a solver that solves this system of constraints.
One condition to optimize on for example is the amount of over-lap
a tile for a iteration has with the tile of a different iteration.
Horn solvers do not appear to solve the problem as is.
However, by looking at the system of constraints, we hope to
find good solutions for these.

Let us formalize this a bit.
Let $L$ be a loop in the program and $L_{i}$ be the $i^{th}$
iteration of the loop. 
Let $Post = \bigwedge \limits_{i=1}^{size} Post_{i}$ be the
assertion/post-condition at the end of this loop.

The non-interference and sliced-property-holds checks can be
done by checking the validity of the Hoare triple 
$\lbrace \bigwedge \limits_{j=1}^{i-1} Post_{j} \rbrace 
L_{i} 
\lbrace \bigwedge \limits_{j=1}^{i} Post_{i} \rbrace$ in
a single go.
However, specifying this in a constraint system is hard as
the number of conjunctions is not known in advance.

Checking non-interference amounts to checking the validity of the Hoare triple 
$\lbrace Post_{i'} \rbrace L_{i} \lbrace Post_{i'} \rbrace$
for $i' < i$.
Similarly, checking sliced-property-holds checks amounts to checking
the validity of the Hoare Triple
$\lbrace Post_{i-1} \rbrace L_{i} \lbrace Post_{i} \rbrace$.
Considering that we will restrict relations in $Post$ to linear arithmetic, 
these checks can be specified as a system of Horn Clauses.
The full range check can also be specified using a system of Horn Clauses.

\subsection{Mid-conditions generation}
A solver that can generate a tile for a given loop in some sense has the
knowledge of loop invariants.
We intend to investigate invariant generation by solving a system of constraints.

Let there be two loops $L_1$ and $L_2$ in the program.
Let the $\forall j \phi'(j) \rightarrow \psi'(j,A)$ be the assertion 
in the given program where $\phi'$ is in linear integer arithmetic
and $\psi'$ is in linear integer arithmetic with theory of arrays.
We want to find the invariant of the form
$\forall j \phi(j) \rightarrow \psi(j,A)$ after the first loop $L_1$.
Then a solution corresponding to the constraint system corresponding 
to the following equation
\begin{align*}
{Pre} \\
Body(L_1) \\
\forall j \phi(j) \rightarrow \psi(j,A) \\
Body(L_2) \\
\forall j \phi'(j) \rightarrow \psi'(j,A)
\end{align*}
along with the system of constraints for tileness checks will generate
the $\phi$ and $\psi$.
This system of constraints relates the invariant to the pre-condition 
of the loop as well as to the assertion in the program.
The hunch is that, this system of constraints is going to be complex,
and hence, we would have to try for each loop instead.


\section{Soundness proof}

A \emph{tiling} of {\A} with respect to {\LL}, $\Inv$ and $\ppost$ is
a binary predicate
$\Tile: \I_{\LL} \times \Ind{\A} \rightarrow \{\ltrue,\lfalse\}$ such
that conditions T1 through T3 listed below hold.  For ease of
notation, we use ``$i^{th}$ tile'' in the discussion below to refer to
all array index values in the set $\{j \mid j \in \Ind{\A} \wedge \Tile(i,
j)\}$.
\begin{itemize}
\item[(T1)] \emph{Full range:} \\
Every array index of interest is present in some tile.  In other
words, the formula $\exists j \in \Ind{\A}\, \forall
i \in \I_{\LL}\, \neg \Tile(i, j)$ must be unsatisfiable.

\item[(T2)] \emph{Sliced post-condition holds inductively:} \\
Recall our post-condition $\ppost \equiv \forall
j \in \Ind{\A}\, \left(\Phi(j) \rightarrow \Psi(\A, j)\right)$.  We define the
sliced post-condition for the $i^{th}$ tile as
$\ppost_i \equiv \forall j \in \Ind{\A}\, \left((\Tile(i,
j) \wedge \Phi(j)) \rightarrow \Psi(\A, j)\right)$.

We now require that if the (possibly weak) loop invariant ${\Inv}$ and
$\bigwedge_{i': i' < i} \ppost_{i'}$ hold prior to
executing the $i^{th}$ loop iteration, then $\ppost_i$ and
${\Inv}$ also hold at the end of the $i^{th}$ loop iteration. In other
words, the Hoare triple $\{\Inv \wedge \bigwedge_{i': i' < i} \ppost_{i'}\} ~~{\LL}_{\mathrm{body}}~~\{\Inv \wedge \ppost_{i}\}$ holds, where ${\LL}_{\mathrm{body}}$
denotes the body of loop ${\LL}$.

\item[(T3)] \emph{Non-interference across tiles:}\\ For $i, i' \in \I_{\LL}$,
if $i' < i$, then loop iteration $i$ does not update any array
element $\A[j]$ which either affects the truth of $\ppost_{i'}$, or for
which $\Tile(i', j)$ holds.
In other words, the Hoare triple 
$\lbrace \Inv \wedge Post_{i'} \rbrace \LL_{i} \lbrace \Inv \wedge Post_{i'} \rbrace$
for all $i' < i$ holds.
This ensures that once we have proved $\{\ppre\}
~~{\LL}~~ \{\bigwedge_{i': i' < i} \ppost_{i'}\}$,
this Hoare triple cannot be violated in the $i^{th}$ as well as any 
subsequent iteration of the loop.
\end{itemize}

\begin{theorem}\label{thm:sound}
Suppose $\Tile: \I_{\LL} \times \Ind{\A} \rightarrow \{\ltrue,\lfalse\}$
satisfies conditions T1 through T3.
If, in addition, $\ppre \rightarrow \Inv$ holds and 
the loop ${\LL}$ iterates at least once, then the Hoare triple 
$\{\ppre\}~~ {\LL}~~ \{\ppost\}$ holds.
\end{theorem}
\begin{proof}
The proof proceeds by induction on the well-founded set $\I_{\LL}$.\\

\textit{Base case:}\\
$i = \LL_{init}$, where $\LL_{init}$ is the initial 
value assigned by the loop.\\
We need to prove $\{\ppre\}~~ {\LL}_{\mathrm{body}} ~~\{\ppost_{i}\}$
holds, where $i = \LL_{init}$.
\begin{align}
&\{\Inv\} ~~{\LL}_{\mathrm{body}}~~\{\Inv \wedge \ppost_{i}\} & (\because T2)\\
&\ppre \rightarrow \Inv & (\because given)\\
&\{\ppre\}~~ {\LL}_{\mathrm{body}} ~~\{\Inv \wedge \ppost_{i}\} & From ~(1)~ \& ~(2)\\
&\{\ppre\}~~ {\LL}_{\mathrm{body}} ~~\{\ppost_{i}\} & (\because 
\Inv \wedge \{\ppost_{i}\} \rightarrow \{\ppost_{i}\} )
\end{align}

\textit{Induction:}\\
Hypothesise that at the beginning of the $i^{th}$ iteration of the loop {\LL} 
the Hoare triple
\begin{align}
& \{\ppre\}~~ {\LL} ~~\{\bigwedge_{i': i' < i}\ppost_{i'}\} & (\because T3)
\end{align}
holds.
Condition T3 ensures that once we have proved $\{\ppre\}
~~{\LL}~~ \{\bigwedge_{i': i' < i} \ppost_{i'}\}$, this Hoare triple
cannot be violated in the $i^{th}$ as well as any subsequent iterations of the loop.
We need to prove that 
$\{\ppre\}~~ {\LL} ~~\{\bigwedge_{i': i' \leq i}\ppost_{i'}\}$ holds.
\begin{align}
& \{\Inv \wedge \bigwedge_{i': i' < i} \ppost_{i'}\} ~~{\LL}_{\mathrm{body}}~~
\{\Inv \wedge \ppost_{i}\} & (\because T2) \\
& \{\Inv \wedge \bigwedge_{i': i' < i} \ppost_{i'}\} ~~{\LL}_{\mathrm{body}}~~
\{\ppost_{i}\} & (\because \Inv \wedge \ppost_{i} \rightarrow \ppost_{i})
\end{align}

At the end of the $i^{th}$ iteration of the loop {\LL} 
the following Hoare triple holds:
\begin{align}
& \{\ppre\}~~ {\LL} ~~\{\bigwedge_{i': i' \leq i}\ppost_{i'}\} & (\because 
From ~(5)~ \& ~(7))
\end{align}

The full range condition says that none of the indices are missed out.
Hence, we can conclude that the conjunction of the post conditions for all the 
iterations gives the post-condition of the loop.
\begin{align}
&\bigwedge_{i \in \I_{\LL}} \ppost_{i} \equiv \ppost & (\because T1)
\end{align}

Thus, from equations (8) \& (9) we conclude that the Hoare triple $\{\ppre\}~~ {\LL}~~ \{\ppost\}$ holds. $\qed$
\end{proof}

\section{Special Cases of Tiles}

\subsection{No tile for some iterations}
Consider the example shown in figure \ref{fig:notile}.

\begin{figure}[h]
{\scriptsize
\begin{verbatim}
  for (i=0; i<SIZE; i++)
  {
    if ( a[i] == b[i] )
    {
      c[j] = i;
      j = j + 1;
    }
  }

  for (k=0; k<j; k++)
  {
    assert(c[k] <= k+i-j);
    assert(c[k] >= k);
  }
\end{verbatim}
}
\label{fig:notile}
\caption{No tile for some iterations}
\end{figure}

The first \textbf{for} loop iterates over all the indices of
array `a' and `b'. It stores `$i$' into the array `c' at
index `$j$' only when the values at index `$i$' in array
`a' and `b' are the same and increments `$j$'.
The assertion states that the value at any index, say `$k$',
in array `c' is less equal `$k+i^*-j^*$', where `$i^*$' and 
`$j^*$' are the values of $i$ and $j$ after the loop terminates. \\

`c' gets modified in the loop, but only in some iterations and not all.
The tile for the $i^{th}$ iteration is $j$, which is a function
of $i$. Such a function may not be obtainable using only the index expressions.
The idea here is to introduce a uninterpreted function, say $f(i)$.
The value of $f(i)$ is constrained by properties such as $a[i] == b[i]$,
$a[i] \neq b[i] \rightarrow f(i) = \bot$, 
$a[i] == b[i] \rightarrow f(i) =$ \textit{previous\_non\_bot\_value} $+ 1$ and so on.
$j$ takes the value $f(i)$ in each iteration.
At the end of the loop, $i^* = SIZE$ and $j^* = f(SIZE)$.
This tile by definition satisfies condition T2(Full Range).
Also note that CBMC works with uninterpreted functions, and hence,
condition T3 can also be checked. Non-interference (T4) holds.
Thus, this example is amenable to proof by tiling.


%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-impl.tex <==
\begin{wrapfigure}[15]{r}{0.4\textwidth}%[h]
\vspace*{-0.9in}
\begin{center}
{\scriptsize
\begin{tikzpicture}
  [
    auto,
    decision/.style = { diamond, draw=black, thick,
                        text width=5em, text badly centered,
                        inner sep=1pt, rounded corners },
    block/.style    = { rectangle, draw=black, very thick,
                        text width=7em, text centered,
                        rounded corners, minimum height=2em },
    line/.style     = { draw, thick, ->, >=stealth, shorten >=0pt },
    dashed/.style     = { draw, thick, dashed, shorten >=0pt },
  ]

  \matrix [column sep=0mm, row sep=3mm] {
    &   \node         (c)    {\textbf{C file}};        &  \\
    &   \node [block] (tran) {\textbf{Transform}};     &  \\
    &   \node [block] (daik) {\textbf{Daikon}};        &  \\
    &   \node [block] (tgen) {\textbf{TileGen}};       &  \\
    &   \node [block] (fel)  {\textbf{For each loop}}; &  \\
    & & \node [block] (ref)  {\textbf{Refine}};           \\
    &   \node [block] (bmc)  {\textbf{TMC}};           &  \\
        \node [block] (res)  {\textbf{Result}};     &  &  \\
  };

  \begin{scope} [every path/.style=line]
    \path (c)          --    (tran);
    \path (tran)       --    (daik);
    \path (daik)       --    (tgen);
    \path (tgen)       --    (fel);
    \path (fel)        --    (bmc);
    \path (bmc.east)   -|    node [near start] {\textbf{Fail}} (ref.south);
    \path (ref.north)  |-    (fel.east);
    \path (bmc.west)   --++  (-0.5,0) node[above, yshift=10mm, rotate=90] {\textbf{Success}} |- ([yshift=-3pt]fel.west);
    \path ([yshift=3pt]fel.west)   -|    (res.north);
  \end{scope}

%  \path (daik.south) -- coordinate (aux) (daik.south|-tgen.north);
%  \draw[dashed] (tgen.north west|-aux) -- (tgen.north east|-aux);    
\end{tikzpicture}
}
\end{center}
\caption{\ourtool~ Tool Diagram}
\label{fig:tool}
\end{wrapfigure}


==> intro.tex <==
Arrays are widely used in programs written in imperative languages.
They are typically used to store large amounts of data of the same
type in an orderly manner in a region of memory that the programmer
views as contiguous, and which she can randomly access by specifying
an index (or offset).  Sequential programs that process large amounts
of data stored in an array commonly use looping constructs to iterate
over the range of array indices of interest and access the
corresponding array elements.  The ease with which data can be
accessed randomly by specifying an index is often exploited by
programmers to access or modify array elements at indices that change
in complex ways within a loop.  While this makes programming easier
when dealing with arrays, it makes reasoning about such programs
harder.  Specifically, the pattern of array accesses within loops can
vary widely from program to program, and may not be easy to infer a
priori.  Furthermore, since the access patterns often span large
regions of the array that depend on program parameters, the array
indices of interest cannot be bounded by statically estimated small
constants.  Hence, reasoning about arrays by treating each array
element as a scalar variable is not a feasible option for analyzing
such programs.  This motivates us to ask if we can automatically infer
program-dependent patterns of array accesses within loops, and use
these patterns to simplify automated verification of programs
manipulating arrays.
%% The combination of the random access and ordered
%% storage makes the automated verification of the array programs
%% particularly hard.

A commonly used approach for formally verifying properties of
sequential programs with loops is to construct an inductive argument.
Typically, we first prove that the desired property is satisfied
before entering a loop for the first time.  We then establish that if
the property is satisfied before entering the loop (at any time),
there is no violation of the property after executing the loop body
once.  This allows us to inductively infer that the property of
interest is satisfied after every iteration of the loop.  A
significant body of research in automated verification is concerned
with the problem of constructing the inductive argument efficiently
for various classes of programs, and there has been remarkable success
in this respect over the last two decades. For programs with loops
manipulating arrays, however, there is an additional complication.
Often, the property of interest at the end of a loop is a universally
quantified statement over all array elements within a specified range
of indices.  Examples of such properties are $\forall i\, \left((0 \le i <
N) \rightarrow (A[i] \geq minVal)\right)$, $\forall i\, \left((0 \le i < N) \wedge
(i \% 2 = 0) \rightarrow (A[i] = i)\right)$, etc.  Interestingly, a single
iteration of the loop may only ensure that the desired property holds
over a limited range of array indices.  Therefore, it is often
necessary to reason about the combination of all loop iterations to
ensure that the quantified property of interest holds at the end of a
loop.  This has important implications for an inductive style of
reasoning.
\begin{itemize}
  \item The quantified property of interest can no longer be used as
    is in an inductive argument, since an individual loop iteration
    may not ensure this property.
  \item We must infer the set of array indices that are used to access
    array elements within a loop iteration, and carve out a ``slice''
    of the quantified property of interest that is relevant for this
    set of indices.  Once this is done, we can apply an inductive
    argument to prove that each loop iteration ensures this slice of
    the property.  Note that this corresponds to understanding access
    patterns of arrays within loops, which can vary significantly from
    one program to another.
  \item We must use compositional reasoning to argue that if each loop
    iteration ensures a slice of the overall property, then the overall
    quantified property holds after the loop terminates.
\end{itemize} 
Our goal in this paper is to design a technique and tool to address
the issues identified above.  %% Our initial experiments suggest that
%% this can yield significant benefits when analyzing programs with
%% varied array access patterns within loops.

%We will be considering a class of programs that use arrays.
%

%% There is an extensive research for the verification of
%% programs with arrays~\cite{booster,arrayfolds,what-decide,cbmc,vaphor}.
%% However, the methods do not perform well on the programs with loops
%% that modify multiple indexes of an array in same iteration.
%% For example, the program in Figure~~\ref{fig:motex}.
%% The multiple updates lead to a large number of cases.
%% To tame the number of cases, the methods attempt to keep the facts
%% about the arrays in a summarized form and join the different cases.
%% Due to the joining, the precise information about the cases is lost.
%% And, the construction of safe inductive invariant fails.

We focus on properties expressed as universally quantified formulas on
arrays, where the quantification is over array indices.  Let $I$
denote a sequence of array index variables and let $A$ denotes an
array used in the program.  For purposes of this paper, we consider
properties of the form $\forall I\, (\Phi(I) \implies \Psi(I, A))$,
where $\Phi(I)$ is a quantifier-free formula in the theory of
integer arithmetic, and $\Psi(I, A)$ is a quantifier-free
formula in the combined theory of arrays and integer arithmetic.
A few examples of such properties were given in the
preceding paragraph.  Note that properties like these are commonly
used to express invariants over arrays after a loop has iterated over
(possibly parts of) the array and performed some computation.  Note
that the restriction on the syntax of the property is motivated by the
ease of carving out ``slices'' of the property for use in an inductive
reasoning.  Significantly, however, the syntactic restriction is
independent of the actual array access patterns in loops within the
program.  Thus, the same property can be used with different loops
having different array access patterns.

%% Specifically, we present an {\em
%%   automated} method that verifies the class of programs against the
%% universal quantified properties,i.e., the properties contain only
%% universal quantifiers and the quantified variables are array indexes.
%% A universal quantified properties looks like $\forall ...( \phi
%% \limplies \psi)$, where $\phi$ is a linear constraints and $\psi$ is a
%% constraints over the array values.

A key contribution of our work is the introduction of the concept of
loop-specific {\em tiles} for analysis of arrays.  As the name
suggests, a tiling partitions the space of relevant array indices into
disjoint parts.  The partitioning is done carefully taking into
account the array access patterns within a loop iteration.  Every tile
thus generated is associated with a unique loop iteration, and a
correct tiling ensures that an iteration of a loop modifies only those
array elements that have indices in the corresponding tile.  This has
several benefits: (i) it helps us obtain loop-specific slices of a
universally quantified property in a straightforward way, (ii) it
helps us combine an inductive proof of a property slice with a
compositional argument that eventually allows us to prove a universally
quantified property of the array, (iii) it allows us to reason
efficiently about programs in which multiple array elements are
modified per iteration, as we will shortly see.
%% %
%% The properties usually refer to a range to indices that are relevant.
%% %
%% If the tiles occurring in the range have corresponding the modification
%% iteration, and they cover the entire range, we have proven
%% that the property holds after the program. 
%% %

We have developed a practical algorithm that automates the process of
tiling.  For simplicity, suppose program under consideration has a
single loop, and the quantified property to be verified is asserted at
the end of the loop.  We introduce a fresh counter variable in the
loop that is incremented in each loop iteration.  This allows us to
uniquely identify an iteration of the loop.  We then use existing
arithmetic invariant generation techniques, viz.~\cite{invgen}, to
identify the relation between indices of array elements accessed in a
loop iteration, and the corresponding loop counter.  This information
is then used to identify a tiling of the array for the loop under
consideration.  More on this is explained later in the paper.
%% We recognize for
%each loop the range of
%% indexes that are modified in each iteration and not modified the
%% future iterations.  By this analysis, we estimate a tiling of each
%% array at each loop.

In a more general scenario, the program under verification may be a
sequence of loops, and the quantified assertion about arrays is
located at the end of the last loop.  In this case, we introduce a
fresh counter variable for each loop, and repeat the same process
independently for each loop to identify the tiling corresponding to
each loop.  Note that a tile corresponding to one loop may be
different from that for another loop, although they turn out to be the
same in most practical examples.  For programs with a sequence of
loops, we also need to infer invariants between loops in order to
compose the tiling-based reasoning for one loop with that for the next
loop in the sequence.  We call such invariants \emph{mid-conditions}.
Since identifying precise invariants is an uncomputable problem, we
work with candidate invariants reported by existing off-the-shelf
annotation/candidate-invariant generators.  Specifically, in our
implementation, we use the dynamic analysis tool
{\daikon}~\cite{daikon} that informs our tool of properties that are
likely (but not proven) to be true between loops.  Our algorithm
checks which of these are provable mid-conditions, and uses only these
to compose the tiling-based reasoning across consecutive loops.  Note
that any other annotation/candidate invariant generator like
{\houdini}~\cite{houdini} could also have been used in place of
{\daikon}, without affecting the soundness of our verification
methodology.

% experimental results
We have implemented our method in a tool called {\ourtool}.  The tool
takes as input a C program with possibly multiple loops in sequence,
and with a universally quantified assertion about arrays at the end of
the last loop.  It automatically generates a tiling of the arrays for
each loop, as described above.  It also uses {\daikon} in a
pre-processing step to generate candidate mid-conditions, and uses
these to come up with a tiling-based compositional proof of the
quantified assertion.  We have applied {\ourtool} on a suite of
benchmarks comprising of several programs that manipulate arrays in
different ways.  {\ourtool} is able to prove the assertion in most of
these benchmarks, whereas several state-of-the-art tools for reasoning
about arrays \vaphor, \booster, and \smackpluscorral~ run out of time
and \cbmc~ runs out of memory on the same benchmarks.
%
% We also observed that the tools we were caught in the case explosion and
% could not summarize the program behaviors. 
%
%\ourtool~outperforms the other tools.
%
Our initial experiments suggest tiling-based compositional reasoning
can be very efficient when reasoning about quantified assertions in a
large class of array manipulating programs.
%

% Our contributions
The primary contributions of the paper can be summarized as follows.
\begin{itemize}
\item We introduce the concept of {\em tiling} for reasoning about
  quantified assertions in programs manipulating arrays in loops.
\item A practical algorithm for verification of a class of array
  programs using tiles
\item A tool implementation that outperforms several state-of-the-art
  tools for reasoning about arrays on a suite of benchmarks.
\end{itemize}
%% One may observe that we use methods like~\daikon~to learn the candidate
%% mid-conditions, which may fail.
%% %
%% However, the search for mid-conditions is guided by the earlier identified
%% tiling.
%% %
%% Therefore, we have more chances of success.
%
%% Since the theory of array is undecidable, a generalized method for
%% reasoning about array manipulating programs cannot be found, and we
%% must focus on techniques that work well on specific classes of
%% programs and/or properties.  In this context, our work is important
%% because it provides a new technique for reasoning about a class of
%% array manipulating programs, for which several state-of-the-art tools
%% seem to face difficulties.  Therefore, using our work in concert with
%% existing techniques for analyzing array manipulating programs is
%% likely to make an ever wider range of array programs amenable to
%% automated analysis.





%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> macro-sup.tex <==
\usepackage{stmaryrd}
\usepackage{hyperref}
\usepackage{mathtools}
% \usepackage[english]{babel}
\usepackage{enumerate}  % enumarate styles
\usepackage{url}
\usepackage[pdftex]{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{galois}
\usepackage{mathabx}
\usepackage{todonotes}
\usepackage{paralist}
\usepackage{multirow}
\usepackage[font=small,skip=0pt]{caption}
\usepackage{subfigure}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{fancyvrb}
\usepackage{lscape}
\usepackage{listings}
\usepackage{pdflscape}
\usepackage{wrapfig}
\usepackage{etoolbox}
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning}
\usetikzlibrary{automata}
\usetikzlibrary{calc}

\lstset{
  basicstyle=\ttfamily,
  mathescape
}

% \lstset{
%   language=C
% }

\sloppy
% comment the following line to bring back the margins
% \IfFileExists{./tmp/rm-margin.tex}{\input{tmp/rm-margin}}{}
% \usepackage[paperheight=19.5cm,paperwidth=12.4cm,margin=.1cm]{geometry}

% \usepackage{algorithm2e}

\makeatletter
\newcommand{\dashedrightarrow}[1][2pt]{%
  \settowidth{\@tempdima}{$\rightarrow$}\rightarrow% typeset arrow
  \makebox[-\@tempdima]{\hskip-1.5ex\color{white}\rule[0.5ex]{#1}{1pt}}% typeset overlay
  \phantom{\rightarrow}% advance appropriate horizontal distance
}
\makeatother

\newcommand{\ashu}[1]{ {\textcolor{magenta} {Ashutosh: #1}} }
\newcommand{\supratik}[1]{ {\textcolor{red} {Supratik: #1}} }
\newcommand{\divesh}[1]{ {\textcolor{blue} {Divyesh: #1}} }

\newcommand{\naturals}{\mathbb{N}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\ordinals}{\mathbb{O}}
\newcommand{\numarals}{\mathbb{I}}

\newtheorem{df}{Definition}
\newcommand{\program}{P}
\newcommand{\sassign}{\;\mathtt{:=}\;}
\newcommand{\defeq}{\triangleq}
\newcommand{\assume}{\mathtt{assume}}
\newcommand{\formulas}{\Sigma}
% \newcommand{\terms}{\mathcal{T}}
\newcommand{\tile}{\tau}

\newcommand{\ppre}{\ensuremath{\mathsf{Pre}}}
\newcommand{\ppost}{\ensuremath{\mathsf{Post}}}
\newcommand{\mexit}[1]{\ensuremath{\mathsf{Cond}_{#1}}}
\newcommand{\ltrue}{\mathbf{tt}}
\newcommand{\lfalse}{\mathbf{ff}}
\newcommand{\limplies}{\Rightarrow}
\newcommand{\lxor}{\oplus}
\newcommand{\Land}{\bigwedge}
\newcommand{\Lor}{\bigvee}
\newcommand{\Lxor}{\bigoplus}
\newcommand{\lequiv}{\Leftrightarrow}
\newcommand{\landplus}{\mathrel{:\hspace{-3pt}\land\hspace{-3pt}=}}
\newcommand{\lorplus}{\mathrel{:\hspace{-3pt}\lor\hspace{-3pt}=}}

\newcommand{\maps}{\rightarrow}

\newcommand{\union}{{\cup} }
\newcommand{\Union}{{\bigcup} }
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\intersection}{{\cap} }
\newcommand{\Intersection}{{\bigcap} }
\newcommand{\compose}{{\circ} }

\newcommand{\locationOf}[1]{loc(#1)}

\newcommand{\formula}{\phi}
\newcommand{\preds}{\pi}
\newcommand{\domain}{\mathcal{D}}

\newcommand{\smem}{\mathcal{S}}
\newcommand{\tout}{TO}


%algorithm names
\newcommand{\concolic}{concolic}

\newcommand{\correct}{\textsc{CORRECT}}

%tool names
% \newcommand{\ourtool}{$\crest^{+}$}
\newcommand{\ourtool}{\textsc{Tiler}}
\newcommand{\zthree}{\textsc{Z3}}
\newcommand{\crest}{\textsc{Crest}}
\newcommand{\synergy}{\textsc{Synergy}}
\newcommand{\cpachecker}{\textsc{CpaChecker}}
\newcommand{\fshell}{\textsc{Fshell}}
\newcommand{\svcomp}{\textsc{SvComp}}
\newcommand{\tiger}{\textsc{CpaTiger}}
\newcommand{\tara}{\textsc{Tara}}
\newcommand{\doublemp}{\mathtt{double\text{-}mp}}
\newcommand{\cbmc}{\textsc{CBMC}}
\newcommand{\booster}{\textsc{Booster}}
\newcommand{\smackpluscorral}{\textsc{SMACK+Corral}}
\newcommand{\corral}{\textsc{Corral}}
\newcommand{\smack}{\textsc{SMACK}}
\newcommand{\houdini}{\textsc{Houdini}}
\newcommand{\boogie}{\textsc{Boogie}}
\newcommand{\invgen}{\textsc{InvGen}}
\newcommand{\clang}{\textsc{Clang}}
\newcommand{\daikon}{\textsc{Daikon}}
\newcommand{\vaphor}{\textsc{Vaphor}}
\newcommand{\spacer}{\textsc{Spacer}}

\newcommand{\musketeer}{\textsc{Musketeer}}
\newcommand{\fender}{\textsc{Fender}}
\newcommand{\blender}{\textsc{Blender}}
\newcommand{\dfence}{\textsc{Dfence}}
\newcommand{\remmex}{\textsc{Remmex}}
\newcommand{\memorax}{\textsc{Memorax}}
\newcommand{\pensieve}{\textsc{Pensieve}}
\newcommand{\trencher}{\textsc{Trencher}}
\newcommand{\persist}{\textsc{Persist}}
\newcommand{\glue}{\textsc{Glue}}

\newcommand{\intel}{\textsc{Intel}}
\newcommand{\arm}{\textsc{ARM}}
\newcommand{\sparc}{\textsc{Sparc}}


\newtheorem{thm}{Theorem}

\newcommand{\rndbr}{RndBr}
\newcommand{\unfrnd}{UnfRnd}
\newcommand{\PP}{\ensuremath{\mathsf P}}
\newcommand{\A}{\ensuremath{\mathsf A}}
\newcommand{\LL}{\ensuremath{\mathsf L}}
\newcommand{\Tile}{\ensuremath{\mathsf Tile}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\Inv}{\ensuremath{\mathsf Inv}}
\newcommand{\Ind}[1]{\ensuremath{\mathsf Index}_{#1}}
%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> new-tiling-copy.tex <==
\begin{algorithm}[!th]
 \caption{\textsc{\ourtool}({\PP} : program, $\ppre$: pre-condition, $\ppost$: post-condition)}
 \label{alg:overall}
\begin{algorithmic}[1]
 \scriptsize
  % \Require 
%%  \State Let $G$ be the CFG for program
%%  ${\PP} = (\mathcal{A}, \mathcal{V}, \mathcal{L}, {\PB})$, as defined in
%%  Section~\ref{sec:prelims}.
%%  %$\mathcal{V}$ = set of non-loop counter scalar variables in P
%% %\Comment{${\PP} = (\mathcal{A}, \mathcal{V}, \mathcal{L}, {\PB})$, as defined in Section~\ref{sec:prelims}}

%% % \State Identify back-edges, cut-points and segments in CFG

%%  {\bf // Initialization}
%%  \State {\CutPoints} := set of cut-points in $G$;
%% %\Comment{Each cut point uniquely identifies a loop}
%%  \State Remove all back-edges from $G$ and topologically sort {\CutPoints};
%%         \Comment{Let $\sqsubseteq$ be the sorted order}
%% % \Comment{ Ensures: if L2 is nested within L1 or L2 is seq composed after L1 within same outer loop, $c2 > c1$}

%% \For{ each $c$ in {\CutPoints} }
%% %   \State loopCtr[$c$] := Unique loop counter of loop corresponding to $c$;
%% %   \State NestLoopCtr[$c$] := Set of loop counters of all loops that nest $c$;
%%    \State CandInv[$c$] := $\emptyset$;
%%    \Comment{Candidate invariant at $c$}
%% \EndFor
%% %\State CommonNestLoopCtrs[entryNode] := CommonNestLoopCtrs[exitNode] := $\emptyset$;
%% \State CandInv[entryNode] := $\ppre$; CandInv[exitNode] := $\ppost$;

%% {\bf // Getting candidate invariants}
%% \For{ each segment $s$ in $G$ from $c_1$ to $c_2$, where $c_1, c_2 \in {\CutPoints} \cup
%%   \{\mathsf{Start}, \mathsf{End}\}$ and $c_1 \sqsubseteq c_2$}
%% %\State CommonNestLoopCtrs[$\mathsf{Start}$] := CommonNestLoopCtrs[$\mathsf{End}$] := $\emptyset$;
%% \State CandInv[$\mathsf{Start}$] := $\ppre$; CandInv[$\mathsf{End}$] := $\ppost$;

%% {\bf // Getting candidate invariants}
%% \For{ each segment s from $c_1$ to $c_2$, where $c_1, c_2 \in {\CutPoints} \cup
%%   \{\mathsf{Start}, \mathsf{End}\}$ and $c_1 \prec c_2$}
%% % to c2 $\in$ (CutPoints $\cup$ {\mathsf{End}}) 
%% %where $c1 < c2$


%% %   \State CommonNestLoopCtrs[s] := NestLoopCtr[c1] $\cap$ NestLoopCtr[c2];
%% %   \If{ (CommonNestLoopCtrs[s] $\neq \emptyset$) }
%%    \If{($s$ lies within a loop)}
%% %      \State $\ell[s]$ := $\min$(CommonNestLoopCtrs);
%% %      \Comment{Loop counter on which we will induct for s}

%%       \State $\ell$[s] := loop counter of innermost nested loop containing $s$;
%% %      \State $\mathsf{OuterVars}$[s] := CommonNestLoopCtrs[s] $\setminus$ $\ell$[s];
%% %      \Comment{Treated as scalar variables that don't change in s}
%%       \State $\mathsf{OuterLoopCtrs}$[s] := loop counters of all other outer loops containing $s$;
%%    \Else  \Comment{ $s$ not in any loop}
%%       \State $\ell$[s] := $\bot$; $\mathsf{OuterLoopCtrs}$[s] := $\emptyset$;
%%    \EndIf
%%   \State $\mathsf{ScalarVars}$[s] := $\mathcal{V} ~\cup~ \mathsf{OuterLoopCtr}$[s];
%%   \State CandInv[$c_2$] := CandInv[$c_2$] $\cup$ findCandInv($c_2$, $s$, $\ell$[s], $\mathsf{ScalarVars}$[s]);
%%   \Comment{findCandInv generates candidate invariants at $c_2$ in terms of $\ell$[s], $\mathsf{ScalarVars}$[s] and arrays in $\mathcal{A}$.}

%% \EndFor
   
%% {\bf // Tiling}
%% \For{each segment $s$ from $c_1$ to $c_2$}
%%     \State ArrayIndexExprsForRead[s] := index expressions used for reading arrays in $s$;
%%     \If{(s lies within a loop)}
%% %
%% %     \For{ each array A accessed in s} \label{T}
%%          \State CandTile[s] := findHeuristicTile(l[s], s); \label{T}
%% %         \State CandOverallTile[s] = CandOverallTile[s] AND CandTile[A][s]
%% %     \EndFor
%%          \State \label{C} Check conditions T1, T2* and T3* for CandTile[s];
%%          \Comment{This requires CandInv[$c_1$], CandInv[$c_2$], ArrayIndexExprsForRead[s] in general};

%%     \If{T1 fails}
%%     \State goto~\ref{T} and re-calculate tiles using different heuristics; 
%%     \EndIf
%%     \If{ T2* or T3* fail}
%%      \State Re-calculate CandInv[$c_1$] and CandInv[$c_2$] using
%%      different heuristics and goto~\ref{C};
%%     \EndIf
%%   \Else \Comment{$s$ not in any loop}
%%   \State
%%    \label{T2} Check modified condition T2*, as described in
%%     Section~\ref{sec:tiling-general};
%%     \If{(check failed)}
%%      \State Re-calculate CandInv[$c_1$] and CandInv[$c_2$] using
%%      different heuristics and goto~\ref{T2};
%%      \EndIf
%%   \EndIf
%% \EndFor
\end{algorithmic}
\end{algorithm}

%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> tiling.tex <==
Consider a program {\PP} with a loop {\LL} that accesses elements of
an array {\A}.  Without loss of generality, we assume that each access
of an element of {\A} in the loop is either a \emph{read access} or
a \emph{write access}.  For example, in the program shown in
Fig.~\ref{fig:simplecode}, the loop {\LL} (lines $3$-$8$) has three
read accesses of {\A} (at lines $3$, $4$ and $5$), and two write
accesses of {\A} (at lines $4$, $5$).  In addition, there are two
write access of {\A} outside the loop {\LL} (at lines $2$ and $9$).
As we will see shortly, write accesses are of crucial importance when
defining tiles.

\begin{wrapfigure}[12]{r}{0.5\textwidth}%[h]
\vspace*{-0.3in}
{\scriptsize
\begin{verbatim}
1. void ArrayUpdate(int A[], int n) {
2.   A[0] = THRESH;
3.   for (int i = 1; i < n-1; i++) { // loop L
4.     if (A[i] < THRESH) { 
5.       A[i+1] = A[i] + 1;
6.       A[i] = A[i-1];
7.     }
8.   }
9.   A[n-1] = THRESH;
10.  // assert(forall i in 0..n, A[i] >= THRESH);
11.   return;
12. }
\end{verbatim}
}
\caption{An array manipulating program}
\label{fig:simplecode}
\end{wrapfigure}
In order to check a universally quantified assertion about the array
at the end of the loop, viz. the assertion in line $10$
of Fig.~\ref{fig:simplecode}, we wish to partition the array based on
how its elements are accessed in different iterations of the loop,
reason about the effect of each loop iteration on the corresponding
segment, and then compose the segment-wise reasoning to prove/disprove
the overall assertion.  %% As we show below, this general recipe works
%% for proving a large class of universally quantified assertions in
%% array manipulating programs.

The above idea of partitioning the array %% based on access patterns in a
%% loop
can be formalized using the notion of \emph{tiles}.  Let {\LL} be
a simple loop that accesses elements of an array {\A}, and for which
the loop exit condition is $\mexit{\LL}$.  We associate a loop counter
$i$ with {\LL}, and assume that $i$ takes values from a well-founded
set of integers $\I_{\LL}$ with $\alpha_{\LL}$ being the minimum
element in the set.  The value of $i$ is assumed to be $\alpha_{\LL}$
in the first iteration of the loop {\LL}, and is incremented in each
subsequent iteration.  Let $\Ind{A}$ denote the set of values of
indices used for accessing elements of {\A} in loop {\LL}. For ease of
exposition, we assume for now that {\A} is a one-dimensional array; we
will shortly see that our ideas generalize to multi-dimensional arrays
as well.

Let $\ppre$ be a pre-condition that holds prior to execution of the
loop.  Let $\ppost$ be an assertion (or post-condition) of the form
$\forall j \in \Ind{\A}\, \left(\Phi(j) \rightarrow \Psi(\A,
j)\right)$ that we wish to verify at the end of loop {\LL}.  The
formula $\Phi(j)$ is assumed to be in the quantifier-free theory of
integer arithmetic, while $\Psi(A, j)$ is assumed to be in the
combined quantifier-free theory of arrays and integer arithmetic.
Note that $\Phi(j)$ restricts the set of values of interest of the
array index $j$, while $\Psi(\A, j)$ describes a desired condition on
the array $\A$, possibly expressed using the index $j$.  Possible
examples of $\Psi(A, j)$ include conditions like $\A[j+1] > j-1$, or
even $\A[j] >= \A[j-1]$.  Let $\Inv$ be a (possibly weak) loop
invariant for loop {\LL}, found by an independent invariant generation
tool.  Clearly, if $\Inv \wedge \neg\mexit{\LL} \rightarrow \ppost$,
then we are already done.  The situation becomes interesting when
$\Inv$ is not strong enough to ensure that
$\Inv \wedge \neg\mexit{\LL} \rightarrow \ppost$.  We encounter
several such cases in our benchmark suite, and it is in these cases
that our method adds value to existing verification flows.

A \emph{tiling} of {\A} with respect to {\LL}, $\Inv$ and $\ppost$ is
a binary predicate
$\Tile: \I_{\LL} \times \Ind{\A} \rightarrow \{\ltrue,\lfalse\}$ such
that conditions T1 through T4 listed below hold.  For ease of
notation, we use ``$i^{th}$ tile'' in the discussion below to refer to
all array index values in the set $\{j \mid j \in \Ind{\A} \wedge \Tile(i,
j)\}$.
\begin{itemize}
\item[(T1)] \emph{Disjointness:} No array index value should be in
tiles corresponding to two different loop counter values.  In other
words, the following formula must be unsatisfiable:~~$\exists i, i' \in
\I_{\LL}\, \exists j \in \Ind{\A}\, (i \neq i') \wedge \Tile(i,
j) \wedge \Tile(i', j)$.

\item[(T2)] \emph{Full range:}
Every array index of interest is present in some tile.  In other
words, the formula $\exists j \in \Ind{\A}\, \forall
i \in \I_{\LL}\, \neg \Tile(i, j)$ must be unsatisfiable.

\item[(T3)] \emph{Sliced post-condition holds inductively:}
Recall our post-condition $\ppost \equiv \forall
j \in \Ind{\A}\, \left(\Phi(j) \rightarrow \Psi(\A, j)\right)$.  We define the
sliced post-condition for the $i^{th}$ tile as
$\ppost_i \equiv \forall j \in \Ind{\A}\, \left((\Tile(i,
j) \wedge \Phi(j)) \rightarrow \Psi(\A, j)\right)$.

We now require that if the (possibly weak) loop invariant ${\Inv}$ and
$\bigwedge_{i': i' < i} \ppost_{i'}$ hold prior to
executing the $i^{th}$ loop iteration, then $\ppost_i$ and
${\Inv}$ also hold at the end of the $i^{th}$ loop iteration. In other
words, the Hoare triple $\{\Inv \wedge \bigwedge_{i': i' < i} \ppost_{i'}\} ~~{\LL}_{\mathrm{body}}~~\{\Inv \wedge \ppost_{i}\}$ holds, where ${\LL}_{\mathrm{body}}$
denotes the body of loop ${\LL}$.

\item[(T4)] \emph{Non-interference across tiles:}  For $i, i' \in \I_{\LL}$,
if $i < i'$, then loop iteration $i'$ does not update any array
element $\A[j]$ which either affects the truth of $\ppost_{i}$, or for
which $\Tile(i, j)$ holds.
\end{itemize}
Note that while tiling depends on $\LL$, $\Inv$ and $\ppost$ in
general, the pattern of array accesses in a loop, i.e $\LL$, often
suggests a natural tiling of array indices that suffices to prove
multiple assertions $\ppost$ using reasonably weak loop invariants
$\Inv$.  The motivating example in Section~\ref{sec:motivating}
illustrates this simplification.

A particularly interesting case of tiling is the example shown in
Fig.~\ref{fig:simplecode}.  In this example, although the $i^{th}$
iteration updates both {\tt A[i]} and {\tt A[i+1]}, the correct choice
of tiling is given by $\Tile(i, j) \equiv (j = i)$.  In fact, if we
(erroneously) choose $\Tile(i, j)$ as $i \le j \le i+1$, condition T1
would be violated, and we would not get a valid tiling.  For this
example, the choice $(j = i)$ satisfies all the required conditions
mentioned above, and is the correct choice of tiling.

\begin{theorem}\label{thm:sound}
Suppose $\Tile: \I_{\LL} \times \Ind{\A} \rightarrow \{\ltrue,\lfalse\}$
satisfies conditions T1 through T4. If, in addition,
$\ppre \rightarrow \Inv$ holds and the loop {\LL} iterates at least
once, then the Hoare triple $\{\ppre\}~~ {\LL}~~ \{\ppost\}$ holds.
\end{theorem}
\noindent \emph{Proof sketch:} The proof proceeds by induction on the
well-founded set $\I_{\LL}$.  The inductive claim is that at the end
of the $i^{th}$ iteration of the loop {\LL}, the Hoare triple
$\{\ppre\}~~ {\LL} ~~\{\bigwedge_{i': i' \leq i}\ppost_{i'}\}$ holds.
The base case is easily seen to be true from condition T3, when $i =
1$.  Condition T4 (and T1) ensure that once we have proved $\{\ppre\}
~~{\LL}~~ \{\bigwedge_{i': i' \leq i} \ppost_{i'}\}$, this Hoare triple
cannot be violated in any subsequent iteration of the loop.  Condition
T3 ensures that the sliced post-condition can be inductively proven
for the $i^{th}$ tile. Since
$\bigwedge_{i \in \I_{\LL}} \ppost_{i} \equiv \ppost$, condition T2
ensures that $\ppost$ indeed holds if {\Inv} holds at the beginning of
the first iteration. This is the compositional step in our approach.
Knowing that $\ppre \rightarrow \Inv$ now allows us to construct a
proof for $\{\ppre\}~~ {\LL}~~ \{\ppost\}$

A few observations are worth noting here.  First, note that there are
no alternation of quantifiers in the check for condition T1, and hence
this check can be easily done by a state-of-the-art SMT solver like
{\zthree}\cite{z3}.  The check for condition T2, however, involves
alternation of quantifiers, and may be hard to check using existing
SMT solvers.

Nevertheless, condition T2 can be simplified if the predicate
$\Tile(i, j)$ is such that whenever $i < i'$, all array indices in
tile $i$ are less than those in tile $i'$.  It turns out that all
tilings that we have encountered in practice have this property. Hence
we conjecture that this is an important class of tiles, and focus only
on such tiles in the subsequent discussion.  For tiles of this class,
the check for T2 is equivalent to the following two checks, each of
which can be done by a state-of-the-art SMT solver.
\begin{itemize}
\item[(T2a)] \emph{Compactness:} This effectively
requires that there be no gaps between consecutive tiles. In other
words, the following formula must be unsatisfiable: $\exists
i \in \I_{\LL} ~\exists j,j',j'' \in \Ind{\A}\,
(i+1 \in \I_{\LL} \wedge \Tile(i, j') \wedge \Tile(i+1,
j'') \wedge \neg \Tile(i,j) \wedge \neg\Tile(i+1,j) \wedge (j' < j <
j''))$.  Significantly, note that there are no alternation of
quantifiers in the formula in this case.
\item[(T2b)] \emph{Inclusion of boundaries:}
Let $\alpha_{\LL}$ and $\beta_{\LL}$ be the minimum and maximum
elements of $\I_{\LL}$.  Similarly, let $\gamma_{\A}$ and
$\delta_{\A}$ be the minimum and maximum elements of $\Ind{\A}$.
Then, we require that $\min \{j : \Tile(\alpha_{\LL}, j) = \ltrue\}
= \gamma_{\A}$ and $\max \{j : \Tile(\beta_{\LL}, j) = \ltrue\}
= \delta_{\A}$.  Since $\Tile$ is defined over
$\I_{\LL} \times \Ind{\A}$, it is easy to see that the above conditions
are equivalent to checking the truth of the formula
$\Tile(\alpha_{\LL}, \gamma_{\A}) \wedge \Tile(\beta_{\LL}, \delta_{\A})$.
\end{itemize}

The check for condition T3 can be done by constructing a program $P'$
that contains a single iteration of the body of loop {\LL}, and by
checking that $\ppost_{i}$ is satisfied after executing the loop body
once, if we start from a state that satisfies ${\Inv} \wedge
\{\bigwedge_{i': i' \leq i} \ppost_{i'}\}$.  If
{\LL} does not have nested loops, this can be formulated as a bounded
model checking problem that can be solved by state-of-the-art bounded
model checkers, viz {\cbmc}~\cite{cbmc}.

Finally, condition T4 can be simplified by requiring the following
conditions:
\begin{itemize}
\item[(T4a)] The $i^{th}$ tile contains exactly the values of array indices
than can be updated in loop iteration $i$.
\item[(T4b)] If $\Tile(i, j) \wedge \Phi(j)$ holds, then the
formula $\Psi(A, j)$ in the sliced post-condition $\ppost$ only refers to
array elements with indices in the $i^{th}$ tile.
\end{itemize}

Note that condition T4a is violated by the choice of tile we made
above for the example in Fig.~\ref{fig:simplecode}.  However, in the
large majority of benchmarks we analyzed, we were able to find tilings
that satisfied condition T4a along with T1, T2 and T3.  The above
discussion shows that while conditions T1, T2, T3 and T4 admit a much
more general definition of tiles, a more restricted definition that
still enjoys all the properties of tiles is obtained by enforcing
conditions T1, T2a, T2b, T3, T4a and T4b.  Indeed, it is easier in
practice to check these new set of conditions that it is to check if
T1, T2, T3 and T4 are satisfied.  Therefore, in our current prototype
implementation, we use conditions T1, T2a, T2b, T3, T4a and T4b.
Conditions T4a and T4b are enforced syntactically by examining the
expressions for indices at all statements in the loop {\LL} where
array updates are made, and in the sliced post-condition.  Checking
conditions T1, T2a and T2b can be done through a state-of-the SMT
solver.  Checking T3 can be done using a state-of-the-art bounded
model checker.

The above discussion was restricted to uni-dimensional arrays.  The
extension to multi-dimensional arrays is straightforward.  Instead of
using one index variable $j$ for accessing arrays, we now allow a
tuple of index variables $(j_1, j_2, \ldots j_r)$ for accessing
arrays.  Each such variable $j_l$ takes values from its own domain,
say $\Ind{\A}^l$.  The entire discussion about tiles above continues
to hold, including the validity of Theorem~\ref{thm:sound}, if we
replace every occurrence of an array index variable $j$ by a sequence
of variables $j_1, \ldots j_r$ and every occurrence of $\Ind{\A}$
$\Ind{\A_1} \times \Ind{\A_2} \ldots \times \Ind{\A_r}$.  We have,
however, restricted ourselves to uni-dimensional arrays for our
implementation and experiments.

%\begin{itemize}
%\item $\Range: 
%\end{itemize}





%% Referring back to the
%% example in Fig.~\ref{fig:simplecode}, both {\tt A[i+1]} and {\tt A[i]}
%% are written in the $i^{th}$ iteration of the loop.  As such

%% A \emph{tiling} for array {\A} with
%% respect to a loop {\LL}
%% c

%\input{alg-tiling}

